Sometimes We Want Translationese

Rapid progress in Neural Machine Translation (NMT) systems over the last few years has been driven primarily towards improving translation quality, and as a secondary focus, improved robustness to input perturbations (e.g. spelling and grammatical mistakes). While performance and robustness are important objectives, by over-focusing on these, we risk overlooking other important properties. In this paper, we draw attention to the fact that for some applications, faithfulness to the original (input) text is important to preserve, even if it means introducing unusual language patterns in the (output) translation. We propose a simple, novel way to quantify whether an NMT system exhibits robustness and faithfulness, focusing on the case of word-order perturbations. We explore a suite of functions to perturb the word order of source sentences without deleting or injecting tokens, and measure the effects on the target side in terms of both robustness and faithfulness. Across several experimental conditions, we observe a strong tendency towards robustness rather than faithfulness. These results allow us to better understand the trade-off between faithfulness and robustness in NMT, and opens up the possibility of developing systems where users have more autonomy and control in selecting which property is best suited for their use case.

==> emnlp2020-templates/Sections/plot.tex <==
\begin{figure*}
    \centering
    \subfigure[]{
        \includegraphics[width=0.4\textwidth]{emnlp2020-templates/graphs/Violin/violin_bleu-4_both_lang.png}
        }
    \subfigure[]{
        \includegraphics[width=0.5\textwidth]{emnlp2020-templates/graphs/Violin/violin_pert_bleu-4_both_pert.png}
        }
    \caption{The general trend of the machine translation systems to favor robust or faithful translations is measured by computing the difference between {\bf faithfulness} and {\bf robustness} scores across languages (a) and perturbations (b). The distributions lying close to $-1$ indicate that the translations to that language or the perturbations are more robust than faithful. Since all languages and all permutations fall to the left of 0.0, we can conclude that NMT models are more robust than they are faithful.}
    \label{fig:violin-plot-main}
\end{figure*}
